Explainable AI Insights for Symbolic Computation: A case study on selecting the variable ordering for cylindrical algebraic decomposition

In recent years there has been increased use of machine learning (ML) techniques within mathematics, including symbolic computation where it may be applied safely to optimise or select algorithms. This paper explores whether using explainable AI (XAI) techniques on such ML models can offer new insight for symbolic computation, inspiring new implementations within computer algebra systems that do not directly call upon AI tools. We present a case study on the use of ML to select the variable ordering for cylindrical algebraic decomposition. It has already been demonstrated that ML can make the choice well, but here we show how the SHAP tool for explainability can be used to inform new heuristics of a size and complexity similar to those human-designed heuristics currently commonly used in symbolic computation.

==> heursitc_charts.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% Please add the following required packages to your document preamble:


\begin{table}[]
\centering
\caption{Heuristic comparison between baseline trained model \cite{florescu2020machine} and balanced dataset created here for the MPL model} 
\label{heurstic_mpl}
\begin{tabular}{l|cc|ccll}
\multicolumn{1}{c|}{\textit{\textbf{MLP}}} & \multicolumn{2}{c|}{\cellcolor[HTML]{E7E6E6}\textbf{Baseline}}                     & \multicolumn{2}{c}{\cellcolor[HTML]{E7E6E6}\textbf{Balanced Data}}                 &  &  \\ \cline{1-5}
\cellcolor[HTML]{E7E6E6}\textbf{Scoring}   & \cellcolor[HTML]{E7E6E6}\textbf{Regular} & \cellcolor[HTML]{E7E6E6}\textbf{Custom} & \cellcolor[HTML]{E7E6E6}\textbf{Regular} & \cellcolor[HTML]{E7E6E6}\textbf{Custom} &  &  \\ \cline{1-5}
\textbf{Best score is}                     & 0.7336                                   & -3.9984                                 & 0.7000                                   & -4.0974                                 &  &  \\
\textbf{warm\_start:}                      & FALSE                                    & FALSE                                   & FALSE                                    & FALSE                                   &  &  \\
\textbf{solver:}                           & lbfgs                                    & lbfgs                                   & lbfgs                                    & lbfgs                                   &  &  \\
\textbf{random\_state:}                    & None                                     & None                                    & None                                     & None                                    &  &  \\
\textbf{learning\_rate:}                   & constant                                 & constant                                & constant                                 & constant                                &  &  \\
\textbf{hidden\_layer\_sizes:}             & 1                                        & 2                                       & {\color[HTML]{FF0000} 2}                 & {\color[HTML]{FF0000} 3}                &  &  \\
\textbf{alpha:}                            & 8.86E-06                                 & 3.79E-05                                & {\color[HTML]{FF0000} 1.44E-06}          & {\color[HTML]{FF0000} 2.98E-06}         &  &  \\
\textbf{activation:}                       & logistic                                 & logistic                                & logistic                                 & logistic                                &  & 
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Heuristic comparison between baseline trained model \cite{florescu2020machine} and balanced dataset created here for the SVC model} 
\label{heurstic_svc}
\begin{tabular}{lccccll}
\multicolumn{1}{c|}{\textit{\textbf{SVC}}}                    & \multicolumn{2}{c|}{\cellcolor[HTML]{E7E6E6}\textbf{Baseline}}                                          & \multicolumn{2}{c}{\cellcolor[HTML]{E7E6E6}\textbf{Balanced Data}}                 &  &  \\ \cline{1-5}
\multicolumn{1}{l|}{\cellcolor[HTML]{E7E6E6}\textbf{Scoring}} & \cellcolor[HTML]{E7E6E6}\textbf{Regular} & \multicolumn{1}{c|}{\cellcolor[HTML]{E7E6E6}\textbf{Custom}} & \cellcolor[HTML]{E7E6E6}\textbf{Regular} & \cellcolor[HTML]{E7E6E6}\textbf{Custom} &  &  \\ \cline{1-5}
\multicolumn{1}{l|}{\textbf{Best Score}}                      & 0.7014                                   & \multicolumn{1}{c|}{-4.0641}                                 & 0.7007                                   & -4.0240                                 &  &  \\
\multicolumn{1}{l|}{\textbf{tol}}                             & 0.0316                                   & \multicolumn{1}{c|}{0.0316}                                  & 0.0316                                   & 0.0316                                  &  &  \\
\multicolumn{1}{l|}{\textbf{Kernel}}                          & rbf                                      & \multicolumn{1}{c|}{rbf}                                     & rbf                                      & rbf                                     &  &  \\
\multicolumn{1}{l|}{\textbf{gamma}}                           & 0.08                                     & \multicolumn{1}{c|}{0.08}                                    & 0.08                                     & 0.08                                    &  &  \\
\multicolumn{1}{l|}{\textbf{C}}                               & 1                                        & \multicolumn{1}{c|}{1}                                       & 1                                        & 1                                       &  &  \\
                                                              & \multicolumn{1}{l}{}                     & \multicolumn{1}{l}{}                                         & \multicolumn{1}{l}{}                     & \multicolumn{1}{l}{}                    &  &  \\
                                                              & \multicolumn{1}{l}{}                     & \multicolumn{1}{l}{}                                         & \multicolumn{1}{l}{}                     & \multicolumn{1}{l}{}                    &  &  \\
                                                              & \multicolumn{1}{l}{}                     & \multicolumn{1}{l}{}                                         & \multicolumn{1}{l}{}                     & \multicolumn{1}{l}{}                    &  & 
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Heuristic comparison between baseline trained model \cite{florescu2020machine} and balanced dataset created here for the decision tree model} 
\label{heurstic_dt}
\begin{tabular}{l|cc|cc}
\multicolumn{1}{c|}{\textit{\textbf{Decision   Tree}}} & \multicolumn{2}{c|}{\cellcolor[HTML]{E7E6E6}\textbf{Baseline}} & \multicolumn{2}{c}{\cellcolor[HTML]{E7E6E6}\textbf{Balanced Data}} \\ \hline
\rowcolor[HTML]{E7E6E6} 
\textbf{Scoring}                                       & \textbf{Regular}              & \textbf{Custom}                & \textbf{Regular}                 & \textbf{Custom}                 \\ \hline
\textbf{Best Score}                                    & \multicolumn{1}{l}{0.7150}    & \multicolumn{1}{l|}{-3.9802}   & \multicolumn{1}{l}{0.6871}       & \multicolumn{1}{l}{-4.1312}     \\
\textbf{Splitter}                                      & best                          & best                           & {\color[HTML]{FF0000} random}    & {\color[HTML]{FF0000} random}   \\
\textbf{max\_depth}                                    & 4                             & 3                              & {\color[HTML]{FF0000} 5}         & {\color[HTML]{FF0000} 5}        \\
\textbf{criterion}                                     & gini                          & gini                           & gini                             & gini                           
\end{tabular}
\end{table}



\begin{table}[]
\centering
\caption{Heuristic comparison between baseline trained model \cite{florescu2020machine} and balanced dataset created here for the knn model} 
\label{heurstic_knn}
\begin{tabular}{l|cc|cc}
\multicolumn{1}{c|}{\textit{\textbf{KNN}}} & \multicolumn{2}{c|}{\cellcolor[HTML]{E7E6E6}\textbf{Baseline}} & \multicolumn{2}{c}{\cellcolor[HTML]{E7E6E6}\textbf{Balanced Data}} \\ \hline
\rowcolor[HTML]{E7E6E6} 
\textbf{Scoring}                           & \textbf{Regular}              & \textbf{Custom}                & \textbf{Regular}                & \textbf{Custom}                  \\ \hline
\textbf{Best Score}                        & \multicolumn{1}{l}{0.7028}    & \multicolumn{1}{l|}{-4.0476}   & \multicolumn{1}{l}{0.6983}      & \multicolumn{1}{l}{-4.0403}      \\
\textbf{Weights}                           & distance                      & distance                       & distance                        & distance                         \\
\textbf{n\_neighbors}                      & 18                            & 18                             & 18                              & 18                               \\
\textbf{algorithm}                         & ball\_tree                    & ball\_tree                     & ball\_tree                      & ball\_tree                      
\end{tabular}
\end{table}

==> top5features_summary.tex <==


\begin{table}[]
\caption{The top five features that each model found to have the highest average impact on model output magnitude. }
\label{top5_all_models}
\begin{tabular}{
>{\columncolor[HTML]{D6DCE4}}c |c
>{\columncolor[HTML]{E7E6E6}}c c
>{\columncolor[HTML]{E7E6E6}}c }
\multicolumn{1}{l|}{\cellcolor[HTML]{8497B0}} & \multicolumn{4}{c}{\cellcolor[HTML]{D6DCE4}\textbf{Model}}                                                                                                                                                                        \\ \hline
\textbf{FI}                 & \multicolumn{1}{c|}{\cellcolor[HTML]{D6DCE4}\textbf{KNN}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D6DCE4}\textbf{MLP}}           & \multicolumn{1}{c|}{\cellcolor[HTML]{D6DCE4}\textbf{SVC}} & \cellcolor[HTML]{D6DCE4}\textbf{DT} \\ \hline
\textbf{1}                                    & \multicolumn{1}{c|}{$avg(max(v_3(S)))$}                & \multicolumn{1}{c|}{\cellcolor[HTML]{E7E6E6}$sum(max(v_3(S)))$}  & \multicolumn{1}{c|}{$avg(max(v_1(S)))$}                & $avg(avg(v_2(S)))$                     \\
\textbf{2}                                    & \multicolumn{1}{c|}{$sum(max(v_3(S)))$}                & \multicolumn{1}{c|}{\cellcolor[HTML]{E7E6E6}$sum(max(v_2(S)))$}  & \multicolumn{1}{c|}{$avg(max(v_2(S)))$}                & $avg(avg(sg(v_1(S)))$                  \\
\textbf{3}                                    & \multicolumn{1}{c|}{$avg(max(v_2(S)))$}                & \multicolumn{1}{c|}{\cellcolor[HTML]{E7E6E6}$sum(avg(v_3(S)))$}  & \multicolumn{1}{c|}{$sum(max(v_2(S)))$}                & $max(sum(v_3(S)))$               \\
\textbf{4}                                    & \multicolumn{1}{c|}{$sum(max(v_2(S)))$}                & \multicolumn{1}{c|}{\cellcolor[HTML]{E7E6E6}$avg(sum(sv_3(S)))$} & \multicolumn{1}{c|}{$avg(max(v_3(S)))$}                & $avg(avg(v_3(S)))$                     \\
\textbf{5}                                    & \multicolumn{1}{c|}{\color[HTML]{643403} \textbf{$max(max(v_1(S)))$}}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{E7E6E6}$sum(avg(v_2(S)))$}  & \multicolumn{1}{c|}{$sum(max(v_3(S)))$}                & $avg(max(v_1(S)))$              
\end{tabular}
\end{table}
